Behind the Veil: Enhanced Indoor 3D Scene Reconstruction with Occluded Surfaces Completion

In this paper, we present a novel indoor 3D reconstruction method with occluded surface completion, given a sequence of depth readings. Prior state-of-the-art (SOTA) methods only focus on the reconstruction of the visible areas in a scene, neglecting the invisible areas due to the occlusions, e.g., the contact surface between furniture, occluded wall and floor. Our method tackles the task of completing the occluded scene surfaces, resulting in a complete 3D scene mesh. The core idea of our method is learning 3D geometry prior from various complete scenes to infer the occluded geometry of an unseen scene from solely depth measurements. We design a coarse-fine hierarchical octree representation coupled with a dual-decoder architecture, i.e., Geo-decoder and 3D Inpainter, which jointly reconstructs the complete 3D scene geometry. The Geo-decoder with detailed representation at fine levels is optimized online for each scene to reconstruct visible surfaces. The 3D Inpainter with abstract representation at coarse levels is trained offline using various scenes to complete occluded surfaces. As a result, while the Geo-decoder is specialized for an individual scene, the 3D Inpainter can be generally applied across different scenes. We evaluate the proposed method on the 3D Completed Room Scene (3D-CRS) and iTHOR datasets, significantly outperforming the SOTA methods by a gain of 16.8% and 24.2% in terms of the completeness of 3D reconstruction. 3D-CRS dataset including a complete 3D mesh of each scene is provided at project webpage.

==> sec/7_3D_CRS.tex <==
%\clearpage
%\setcounter{page}{1}
%\maketitlesupplementary

\section{3D-CRS Dataset}
\label{subsection8}
%
\begin{figure*}[!h]
    \centering
    \includegraphics[width=1.0\textwidth]{figures/3D-CRS-data.pdf}
    \caption{ Some examples of 2D rendered data from the 3D-CRS dataset: showcasing from left to right, RGB, depth, semantic mask, normal and albedo. We only use depth images and 3D meshes in the experiment of this manuscript.
    }
  \label{fig:CRS-data}
\end{figure*}
%
\begin{figure*}[!h]
    \centering
    \includegraphics[width=1.0\textwidth]{figures/furniture_meshes.pdf}
    \caption{Some examples of complete 3D furniture mesh from the 3D-CRS dataset. 
    }
  \label{fig:furniture_meshes}
\end{figure*}
%
\begin{figure*}[!h]
    \centering
    \includegraphics[width=1.0\textwidth]{figures/scene_mesh_new.pdf}
    \caption{Some examples of complete 3D scene mesh (left), 3D room layout mesh (middle) and 3D scene model (right) from the 3D-CRS dataset.
    }
  \label{fig:scene_meshes}
  \vspace{-5mm}
\end{figure*}
%
To address the limitations of existing public indoor RGB-D datasets, which typically lack complete 3D meshes of room scenes and furniture, we build a novel dataset, named the 3D Complete Room Scene (3D-CRS) upon a commercial indoor 3D dataset provided by Coohome LLC~\footnote{\url{https://www.coohom.com/b2b}}.
% Although the scene dataset from AI2-THOR~\cite{ai2thor} includes complete 3D scene meshes, the photorealistic quality of their data does not meet high-quality standards, and the complexity of their room layouts is insufficient.
Although the scene dataset from AI2-THOR~\cite{ai2thor} includes complete 3D scene meshes, their data does not meet the high-quality photorealistic standards, and the complexity of their room layouts is insufficient.
Consequently. we created the 3D-CRS dataset to facilitate further research on 3D surface completion. 
The 3D-CRS dataset, illustrated in Figure~\ref{fig:scene_meshes}: right, is meticulously crafted by 3D artists using Unreal Engine 4.27. 
It features 20 high-quality indoor scenarios that represent typical household rooms, including kitchens, bathrooms, living rooms, and bedrooms. 
We utilized the virtual camera in Unreal Engine to render an extensive amount of photorealistic data from these high-quality 3D scene models. 
The camera trajectory is determined using Catmull-Rom spline interpolation, based on a series of manually selected control points, aiming to encompass the majority space of each room scene.
We render 2D images at $1024 \times 768$ resolution using a 120-degree FOV camera along the camera trajectory, under the automatic exposure and default indoor light in Unreal Engine.
As shown in Figure~\ref{fig:CRS-data}, each scene in the 3D-CRS dataset includes RGB images, depth images, normal images, semantic/instance masks, and albedo. 
Besides the 2D rendering data, we also provide the complete 3D scene meshes (Figure~\ref{fig:scene_meshes}: left) for each room, consisting of both complete 3D furniture meshes (Figure~\ref{fig:furniture_meshes}) and complete 3D room layout meshes (Figure~\ref{fig:scene_meshes}: middle). 
The 3D-CRS dataset's configuration allows AI agents to interact with objects in these environments in various ways. 
Our 3D scene models are designed to be seamlessly compatible with robotics simulations, such as NVIDIA's Isaac Sim\footnote{https://developer.nvidia.com/isaac-sim}.
Our 3D-CRS dataset greatly enhances the potential for research in 3D surface completion and other robotics-related fields.
